A latent variable approach to account for correlated inputs in global sensitivity analysis with cases from pharmacological systems modelling

In pharmaceutical research and development decision-making related to drug candidate selection, efficacy and safety is commonly supported through modelling and simulation (M\&S). Among others, physiologically-based pharmacokinetic models are used to describe drug absorption, distribution and metabolism in human. Global sensitivity analysis (GSA) is gaining interest in the pharmacological M\&S community as an important element for quality assessment of model-based inference. Physiological models often present inter-correlated parameters. The inclusion of correlated factors in GSA and the sensitivity indices interpretation has proven an issue for these models. Here we devise and evaluate a latent variable approach for dealing with correlated factors in GSA. This approach describes the correlation between two model inputs through the causal relationship of three independent factors: the latent variable and the unique variances of the two correlated parameters. Then, GSA is performed with the classical variance-based method. We applied the latent variable approach to a set of algebraic models and a case from physiologically-based pharmacokinetics. Then, we compared our approach to Sobol's GSA assuming no correlations, Sobol's GSA with groups and the Kucherenko approach. The relative ease of implementation and interpretation makes this a simple approach for carrying out GSA for models with correlated input factors.

==> bibliography.tex <==
\begin{thebibliography}{10}
	
	\bibitem{chmp_ema_guideline_2018}
	{CHMP (EMA)}.
	\newblock Guideline on the reporting of physiologically based pharmacokinetic
	({PBPK}) modelling and simulation.
	\newblock Technical Report EMA/CHMP/458101/2016, Committee for Medicinal
	Products for Human Use (CHMP), European Medicines Agency (EMA), London, UK,
	December 2018.
	
	\bibitem{fda_pbpkguide_2018}
	CDER.
	\newblock Physiologically based pharmacokinetic analyses - format and content:
	Guidance for industry, 2018.
	
	\bibitem{melillo_variance_2019}
	Nicola Melillo, Leon Aarons, Paolo Magni, and Adam~S. Darwich.
	\newblock Variance based global sensitivity analysis of physiologically based
	pharmacokinetic absorption models for bcs i-iv drugs.
	\newblock {\em Journal of Pharmacokinetics and Pharmacodynamics}, 46(1):27--42,
	February 2019.
	
	\bibitem{melillo_accounting_2019}
	Nicola Melillo, Adam~S. Darwich, Paolo Magni, and Amin Rostami-Hodjegan.
	\newblock Accounting for inter-correlation between enzyme abundance: a
	simulation study to assess implications on global sensitivity analysis within
	physiologically-based pharmacokinetics.
	\newblock {\em Journal of Pharmacokinetics and Pharmacodynamics},
	46(2):137--154, April 2019.
	
	\bibitem{melillo_inter-compound_2020}
	Nicola Melillo, Silvia Grandoni, Nicola Cesari, Giandomenico Brogin, Paola
	Puccini, and Paolo Magni.
	\newblock Inter-compound and {Intra}-compound {Global} {Sensitivity} {Analysis}
	of a {Physiological} {Model} for {Pulmonary} {Absorption} of {Inhaled}
	{Compounds}.
	\newblock {\em The AAPS Journal}, 22(5):116, August 2020.
	
	\bibitem{mcnally_workflow_2011}
	Kevin McNally, Richard Cotton, and George~D. Loizou.
	\newblock A {Workflow} for {Global} {Sensitivity} {Analysis} of {PBPK}
	{Models}.
	\newblock {\em Frontiers in Pharmacology}, 2:31, 2011.
	
	\bibitem{zhang_sobol_2015}
	X-Y Zhang, Mn~Trame, Lj~Lesko, and S~Schmidt.
	\newblock Sobol {Sensitivity} {Analysis}: {A} {Tool} to {Guide} the
	{Development} and {Evaluation} of {Systems} {Pharmacology} {Models}.
	\newblock {\em CPT: Pharmacometrics \& Systems Pharmacology}, 4(2):69--79,
	February 2015.
	
	\bibitem{daga_physiologically_2018-1}
	Pankaj~R. Daga, Michael~B. Bolger, Ian~S. Haworth, Robert~D. Clark, and Eric~J.
	Martin.
	\newblock Physiologically {Based} {Pharmacokinetic} {Modeling} in {Lead}
	{Optimization}. 2. {Rational} {Bioavailability} {Design} by {Global}
	{Sensitivity} {Analysis} {To} {Identify} {Properties} {Affecting}
	{Bioavailability}.
	\newblock {\em Molecular Pharmaceutics}, 15(3):831--839, March 2018.
	
	\bibitem{yau_gsappkrr_2020}
	E.~Yau, A.~Olivares-Morales, M.~Gertz, N.~Parrott, A.~S. Darwich, L.~Aarons,
	and K.~Ogungbenro.
	\newblock Global sensitivity analysis of the rodgers and rowland model for
	prediction of tissue: Plasma partitioning coefficients: Assessment of the key
	physiological and physicochemical factors that determine small-molecule
	tissue distribution.
	\newblock {\em AAPS J}, 22(2):41, 2020.
	
	\bibitem{liu_investigating_2019}
	Dan Liu, Linzhong Li, Amin Rostami-Hodjegan, and Masoud Jamei.
	\newblock Investigating {Impacts} of {Model} {Parameters} {Correlations} in
	{Global} {Sensitivity} {Analysis}: {Determining} the most influential
	parameters of a {Minimal} {PBPK} {Model} of {Midazolam}.
	\newblock In {\em PAGE 28, Abstr 8875 [www.page-meeting.org/?abstract=8875]},
	Stockholm, Sweden, 2019.
	
	\bibitem{efpia_mid3goodpractices_2016}
	EFPIA~MID3 Workgroup, SF~Marshall, R~Burghaus, V~Cosson, SYA Cheung, M~Chenel,
	O~DellaPasqua, N~Frey, B~HamrÃ©n, L~Harnisch, F~Ivanow, T~Kerbusch,
	J~Lippert, PA~Milligan, S~Rohou, A~Staab, JL~Steimer, C~TornÃ¸e, and SAG
	Visser.
	\newblock Good practices in model-informed drug discovery and development:
	Practice, application, and documentation.
	\newblock {\em CPT: Pharmacometrics \& Systems Pharmacology}, 5(3):93--122,
	2016.
	
	\bibitem{saltelli_what_2013}
	Andrea Saltelli, \^Angela Guimaraes~Pereira, Jeroen P. Van~der Sluijs, and
	Silvio Funtowicz.
	\newblock What do {I} make of your latinorum? {Sensitivity} auditing of
	mathematical modelling.
	\newblock {\em International Journal of Foresight and Innovation Policy},
	9(2/3/4):213, 2013.
	
	\bibitem{aarons_physiologically_2005}
	L.~Aarons.
	\newblock Physiologically based pharmacokinetic modelling: a sound mechanistic
	basis is needed.
	\newblock {\em British Journal of Clinical Pharmacology}, 60(6):581--583, 2005.
	\newblock \_eprint:
	https://bpspubs.onlinelibrary.wiley.com/doi/pdf/10.1111/j.1365-2125.2005.02560.x.
	
	\bibitem{bonate_poppkpd_2005}
	P.~L. Bonate.
	\newblock Recommended reading in population pharmacokinetic pharmacodynamics.
	\newblock {\em AAPS J}, 7(2):E363--73, 2005.
	
	\bibitem{jones_basic_2013}
	H.~M. Jones and K.~Rowland-Yeo.
	\newblock Basic {Concepts} in {Physiologically} {Based} {Pharmacokinetic}
	{Modeling} in {Drug} {Discovery} and {Development}.
	\newblock {\em CPT: Pharmacometrics \& Systems Pharmacology}, page~63, 2013.
	
	\bibitem{sasso_pbtk_2010}
	A.~F. Sasso, S.~S. Isukapalli, and P.~G. Georgopoulos.
	\newblock A generalized physiologically-based toxicokinetic modeling system for
	chemical mixtures containing metals.
	\newblock {\em Theor Biol Med Model}, 7:17, 2010.
	
	\bibitem{nestorov_wbpbpk_2007}
	I.~Nestorov.
	\newblock Whole-body physiologically based pharmacokinetic models.
	\newblock {\em Expert Opin Drug Metab Toxicol}, 3(2):235--49, 2007.
	
	\bibitem{jamei_pbpklabel_2016}
	Masoud Jamei.
	\newblock Recent advances in development and application of
	physiologically-based pharmacokinetic (pbpk) models: a transition from
	academic curiosity to regulatory acceptance.
	\newblock {\em Current pharmacology reports}, 2:161--169, 2016.
	
	\bibitem{grimstein_physiologically_2019}
	Manuela Grimstein, Yuching Yang, Xinyuan Zhang, Joseph Grillo, Shiew-Mei Huang,
	Issam Zineh, and Yaning Wang.
	\newblock Physiologically {Based} {Pharmacokinetic} {Modeling} in {Regulatory}
	{Science}: {An} {Update} {From} the {U}.{S}. {Food} and {Drug}
	{Administration}'s {Office} of {Clinical} {Pharmacology}.
	\newblock {\em Journal of Pharmaceutical Sciences}, 108(1):21--25, January
	2019.
	
	\bibitem{tsamandouras_incorporation_2015}
	Nikolaos Tsamandouras, Thierry Wendling, Amin Rostami-Hodjegan, Aleksandra
	Galetin, and Leon Aarons.
	\newblock Incorporation of stochastic variability in mechanistic population
	pharmacokinetic models: handling the physiological constraints using normal
	transformations.
	\newblock {\em Journal of Pharmacokinetics and Pharmacodynamics},
	42(4):349--373, August 2015.
	
	\bibitem{rostamihodjegan_reverse_2018}
	Amin Rostami-Hodjegan.
	\newblock Reverse {Translation} in {PBPK} and {QSP}: {Going} {Backwards} in
	{Order} to {Go} {Forward} {With} {Confidence}.
	\newblock {\em Clinical Pharmacology \& Therapeutics}, 103(2):224--232, 2018.
	
	\bibitem{bai_omicspharmaceutics_2018}
	Jane P.~F. Bai, Ioannis~N. Melas, Junguk Hur, and Ellen Guo.
	\newblock Advances in omics for informed pharmaceutical research and
	development in the era of systems medicine.
	\newblock {\em Expert Opinion on Drug Discovery}, 13(1):1--4, 2018.
	\newblock PMID: 29073782.
	
	\bibitem{doki_pbpkcorr_2018}
	Kosuke Doki, Adam~S. Darwich, Brahim Achour, Aleksi Tornio, Janne~T. Backman,
	and Amin Rostami-Hodjegan.
	\newblock Implications of intercorrelation between hepatic cyp3a4-cyp2c8
	enzymes for the evaluation of drug-drug interactions: a case study with
	repaglinide.
	\newblock {\em British journal of clinical pharmacology}, 84(5):972--986, 2018.
	
	\bibitem{garciacremades_mechanistic_2020}
	Maria Garcia Cremades, Nicola Melillo, Inaki~F. Troconiz, and Paolo Magni.
	\newblock Mechanistic {Multiscale} {Pharmacokinetic} {Model} for the
	{Anticancer} {Drug} Gemcitabine in
	{Pancreatic} {Cancer}.
	\newblock {\em Clinical and Translational Science}, XX, 2020.
	
	\bibitem{rowland_pbpkdrivers_2018}
	A.~Rowland, M.~van Dyk, A.~M. Hopkins, R.~Mounzer, T.~M. Polasek,
	A.~Rostami-Hodjegan, and M.~J. Sorich.
	\newblock Physiologically based pharmacokinetic modeling to identify
	physiological and molecular characteristics driving variability in drug
	exposure.
	\newblock {\em Clin Pharmacol Ther}, 104(6):1219--1228, 2018.
	
	\bibitem{sobol_sensitivity_1993}
	Ilya~M. Sobol.
	\newblock Sensitivity {Estimates} for {Nonlinear} {Mathematical} {Models}.
	\newblock {\em Mathematical modelling and computational experiments},
	1(4):407--414, 1993.
	
	\bibitem{saltelli_making_2002}
	Andrea Saltelli.
	\newblock Making best use of model evaluations to compute sensitivity indices.
	\newblock {\em Computer Physics Communications}, 145(2):280--297, May 2002.
	
	\bibitem{saltelli_global_2008}
	Andrea Saltelli, Marco Ratto, Terry Andres, Francesca Campolongo, Jessica
	Cariboni, Debora Gatelli, Michaela Saisana, and Stefano Tarantola.
	\newblock {\em Global {Sensitivity} {Analysis}. {The} {Primer}}.
	\newblock John Wiley \& Sons, Ltd, January 2008.
	
	\bibitem{oakley_probabilistic_2004}
	Jeremy~E. Oakley and Anthony O'Hagan.
	\newblock Probabilistic sensitivity analysis of complex models: a {Bayesian}
	approach.
	\newblock {\em Journal of the Royal Statistical Society: Series B (Statistical
		Methodology)}, 66(3):751--769, 2004.
	\newblock \_eprint:
	https://rss.onlinelibrary.wiley.com/doi/pdf/10.1111/j.1467-9868.2004.05304.x.
	
	\bibitem{iooss_shapley_2019}
	Bertrand Iooss and Clementine Prieur.
	\newblock Shapley effects for sensitivity analysis with correlatedinputs:
	comparisons with {Sobol} indices, numericalestimation and applications.
	\newblock {\em International Journal for Uncertainty Quantification}, 9(5),
	2019.
	\newblock Publisher: Begel House Inc.
	
	\bibitem{liu_considerations_2020}
	Dan Liu, Linzhong Li, Amin Rostami-Hodjegan, Frederic~Y. Bois, and Masoud
	Jamei.
	\newblock Considerations and {Caveats} when {Applying} {Global} {Sensitivity}
	{Analysis} {Methods} to {Physiologically} {Based} {Pharmacokinetic} {Models}.
	\newblock {\em The AAPS Journal}, 22(5):93, July 2020.
	
	\bibitem{mara_nonparam_2015}
	Thierry~A. Mara, Stefano Tarantola, and Paola Annoni.
	\newblock Non-parametric methods for global sensitivity analysis of model
	output with dependent inputs.
	\newblock {\em Environmental Modelling \& Software}, 72:173 -- 183, 2015.
	
	\bibitem{do_correlation_2020}
	Nhu~Cuong Do and Saman Razavi.
	\newblock Correlation {Effects}? {A} {Major} but {Often} {Neglected}
	{Component} in {Sensitivity} and {Uncertainty} {Analysis}.
	\newblock {\em Water Resources Research}, 56(3):e2019WR025436, 2020.
	\newblock \_eprint:
	https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2019WR025436.
	
	\bibitem{da_veiga_local_2009}
	Sebastien Da~Veiga, Francois Wahl, and Fabrice Gamboa.
	\newblock Local {Polynomial} {Estimation} for {Sensitivity} {Analysis} on
	{Models} {With} {Correlated} {Inputs}.
	\newblock {\em Technometrics}, 51(4):452--463, November 2009.
	
	\bibitem{li_global_2010}
	Genyuan Li, Herschel Rabitz, Paul~E. Yelvington, Oluwayemisi~O. Oluwole, Fred
	Bacon, Charles~E. Kolb, and Jacqueline Schoendorf.
	\newblock Global {Sensitivity} {Analysis} for {Systems} with {Independent}
	and/or {Correlated} {Inputs}.
	\newblock {\em The Journal of Physical Chemistry A}, 114(19):6022--6032, May
	2010.
	
	\bibitem{xu_extending_2007}
	C.~Xu and G.~Gertner.
	\newblock Extending a global sensitivity analysis technique to models with
	correlated parameters.
	\newblock {\em Computational Statistics \& Data Analysis}, 51(12):5579--5590,
	August 2007.
	
	\bibitem{kucherenko_estimation_2012}
	S.~Kucherenko, S.~Tarantola, and P.~Annoni.
	\newblock Estimation of global sensitivity indices for models with dependent
	variables.
	\newblock {\em Computer Physics Communications}, 183(4):937--946, April 2012.
	
	\bibitem{tarantola_variance-based_2017}
	S.~Tarantola and Thierry~A. Mara.
	\newblock {Variance}-{based} {sensitivity} {indices} {of} {computer} {models}
	{with} {dependent} {inputs}: {the} {Fourier} {amplitude} {sensitivity}
	{test}.
	\newblock {\em International Journal for Uncertainty Quantification}, 7(6),
	2017.
	\newblock Publisher: Begel House Inc.
	
	\bibitem{noauthor_simcyp_2019}
	CERTARA L.P.
	\newblock Simcyp {Simulator} - {Version} 19, 2019.
	
	\bibitem{borgonovo_sensitivity_2016}
	Emanuele Borgonovo and Elmar Plischke.
	\newblock Sensitivity analysis: {A} review of recent advances.
	\newblock {\em European Journal of Operational Research}, 248(3):869--887,
	February 2016.
	
	\bibitem{pianosi_sensitivity_2016}
	Francesca Pianosi, Keith Beven, Jim Freer, Jim~W. Hall, Jonathan Rougier,
	David~B. Stephenson, and Thorsten Wagener.
	\newblock Sensitivity analysis of environmental models: {A} systematic review
	with practical workflow.
	\newblock {\em Environmental Modelling \& Software}, 79:214--232, May 2016.
	
	\bibitem{iooss_review_2015}
	Bertrand Iooss and Paul LemaÃƒÂ®tre.
	\newblock A {Review} on {Global} {Sensitivity} {Analysis} {Methods}.
	\newblock In {\em Uncertainty {Management} in {Simulation}-{Optimization} of
		{Complex} {Systems}}, Operations {Research}/{Computer} {Science} {Interfaces}
	{Series}, pages 101--122. Springer, Boston, MA, 2015.
	
	\bibitem{kostewicz_pbpksoftware_2014}
	E.~S. Kostewicz, L.~Aarons, M.~Bergstrand, M.~B. Bolger, A.~Galetin, O.~Hatley,
	M.~Jamei, R.~Lloyd, X.~Pepin, A.~Rostami-Hodjegan, E.~Sjogren, C.~Tannergren,
	D.~B. Turner, C.~Wagner, W.~Weitschies, and J.~Dressman.
	\newblock Pbpk models for the prediction of in vivo performance of oral dosage
	forms.
	\newblock {\em Eur J Pharm Sci}, 57:300--21, 2014.
	
	\bibitem{loehlin_latent_2017}
	John~C. Loehlin and A.~Alexander Beaujean.
	\newblock {\em Latent {Variable} {Models}: {An} {Introduction} to {Factor},
		{Path}, and {Structural} {Equation} {Analysis}}.
	\newblock Routledge, New York, fifth edition edition, 2017.
	
	\bibitem{brown_confirmatory_2015}
	Timothy~A. Brown.
	\newblock {\em Confirmatory {Factor} {Analysis} for {Applied} {Research}}.
	\newblock Guilford Press, New York, second edition edition, January 2015.
	
	\bibitem{Galetin_midazolam_2004}
	Aleksandra Galetin, Caroline Brown, David Hallifax, Kiyomi Ito, and J.~Brian
	Houston.
	\newblock Utility of recombinant enzyme kinetics in prediction of human
	clearance: Impact of variability, cyp3a5, and cyp2c19 on cyp3a4 probe
	substrates.
	\newblock {\em Drug Metabolism and Disposition}, 32(12):1411--1420, 2004.
	
	\bibitem{roy_cyp3a5polymorphism_2005}
	J.~N. Roy, J.~Lajoie, L.~S. Zijenah, A.~Barama, C.~Poirier, B.~J. Ward, and
	M.~Roger.
	\newblock Cyp3a5 genetic polymorphisms in different ethnic populations.
	\newblock {\em Drug Metab Dispos}, 33(7):884--7, 2005.
	
	\bibitem{lolodi_pxrcyp3a_2017}
	O.~Lolodi, Y.~M. Wang, W.~C. Wright, and T.~Chen.
	\newblock Differential regulation of cyp3a4 and cyp3a5 and its implication in
	drug discovery.
	\newblock {\em Curr Drug Metab}, 18(12):1095--1105, 2017.
	
	\bibitem{homma_importance_1996}
	Toshimitsu Homma and Andrea Saltelli.
	\newblock Importance measures in global sensitivity analysis of nonlinear
	models.
	\newblock {\em Reliability Engineering \& System Safety}, 52(1):1--17, April
	1996.
	
	\bibitem{farrell_ave_2009}
	Andrew~M. Farrell.
	\newblock Insufficient discriminant validity: A comment on bove, pervan,
	beatty, and shiu (2009).
	\newblock {\em Journal of Business Research}, 63(3):324 -- 327, 2010.
	
	\bibitem{fornell_evaluating_1981}
	Claes Fornell and David~F. Larcker.
	\newblock Evaluating {Structural} {Equation} {Models} with {Unobservable}
	{Variables} and {Measurement} {Error}.
	\newblock {\em Journal of Marketing Research}, 18(1):39--50, 1981.
	\newblock Publisher: American Marketing Association.
	
	\bibitem{berezhkovskiy_valid_2010}
	Leonid~M. Berezhkovskiy.
	\newblock A {Valid} {Equation} for the {Well}-{Stirred} {Perfusion} {Limited}
	{Physiologically} {Based} {Pharmacokinetic} {Model} that {Consistently}
	{Accounts} for the {Blood}â€“{Tissue} {Drug} {Distribution} in the {Organ}
	and the {Corresponding} {Valid} {Equation} for the {Steady} {State} {Volume}
	of {Distribution}.
	\newblock {\em Journal of Pharmaceutical Sciences}, 99(1):475--485, January
	2010.
	
	\bibitem{vossen_dynamically_2007}
	Michaela Vossen, Michael Sevestre, Christoph Niederalt, In-Jin Jang, Stefan
	Willmann, and Andrea~N. Edginton.
	\newblock Dynamically simulating the interaction of midazolam and the {CYP3A4}
	inhibitor itraconazole using individual coupled whole-body
	physiologically-based pharmacokinetic ({WB}-{PBPK}) models.
	\newblock {\em Theoretical Biology and Medical Modelling}, 4(1):13, March 2007.
	
	\bibitem{michaelis_kinetik_1913}
	{Michaelis L.} and {Menten M.L.}
	\newblock Die {Kinetik} der {Invertinwirkung}.
	\newblock {\em Biochemistry Zeitung}, 49:333 -- 369, 1913.
	
	\bibitem{rostamihodjegan_simulation_2007}
	Amin Rostami-Hodjegan and Geoffrey~T. Tucker.
	\newblock Simulation and prediction of in vivo drug metabolism in human
	populations from in vitro data.
	\newblock {\em Nature Reviews Drug Discovery}, 6(2):140--148, February 2007.
	\newblock Number: 2 Publisher: Nature Publishing Group.
	
	\bibitem{rowland_clinical_1995}
	Malcolm Rowland and Thomas~N. Tozer.
	\newblock {\em Clinical {Pharmacokinetics}: {Concepts} and {Applications}}.
	\newblock Lippincott Williams \& Wilkins, third edition, 1995.
	
	\bibitem{cacciari_italian_2006}
	E.~Cacciari, S.~Milani, A.~Balsamo, E.~Spada, G.~Bona, L.~Cavallo, F.~Cerutti,
	L.~Gargantini, N.~Greggio, G.~Tonini, and A.~Cicognani.
	\newblock Italian cross-sectional growth charts for height, weight and {BMI} (2
	to 20 yr).
	\newblock {\em Journal of Endocrinological Investigation}, 29(7):581--593, July
	2006.
	
	\bibitem{WHO:BMI}
	World Health~Organization (WHO).
	\newblock {\em Body Mass Index - BMI, (accessed September 28, 2020)}, 2020.
	\newblock
	\url{https://www.euro.who.int/en/health-topics/disease-prevention/nutrition/a-healthy-lifestyle/body-mass-index-bmi}.
	
	\bibitem{cubitt_sources_2011}
	Helen~E. Cubitt, Karen~R. Yeo, Eleanor~M. Howgate, Amin Rostami-Hodjegan, and
	Zoe~E. Barter.
	\newblock Sources of interindividual variability in {IVIVE} of clearance: an
	investigation into the prediction of benzodiazepine clearance using a
	mechanistic population-based pharmacokinetic model.
	\newblock {\em Xenobiotica}, 41(8):623--638, August 2011.
	\newblock Publisher: Taylor \& Francis \_eprint:
	https://doi.org/10.3109/00498254.2011.560294.
	
	\bibitem{noauthor_simcyp_2017}
	CERTARA L.P.
	\newblock Simcyp {Simulator} - {Version} 17, April 2017.
	
	\bibitem{achour_simultaneous_2014}
	Brahim Achour, Matthew~R. Russell, Jill Barber, and Amin Rostami-Hodjegan.
	\newblock Simultaneous {Quantification} of the {Abundance} of {Several}
	{Cytochrome} {P}450 and {Uridine} 5'-{Diphospho}-{Glucuronosyltransferase}
	{Enzymes} in {Human} {Liver} {Microsomes} {Using} {Multiplexed} {Targeted}
	{Proteomics}.
	\newblock {\em Drug Metabolism and Disposition}, 42(4):500--510, April 2014.
	
	\bibitem{noauthor_matlab_2019}
	The {M}athWorks.
	\newblock {MATLAB} {R}2019b, the {M}ahworks, inc., {N}atick, {M}assachusetts,
	{U}nited {S}tates, 2019.
	
	\bibitem{Marelli_uqlab_2014}
	S.~Marelli and B.~Sudret.
	\newblock {UQLab}: a framework for uncertainty quantification in {MATLAB}.
	\newblock In {\em Proc. 2nd Int. Conf. on Vulnerability, Risk Analysis and
		Management {(ICVRAM2014)}, Liverpool, United Kingdom}, 2014.
	
	\bibitem{meek_case_2013}
	M.~E.~(Bette) Meek, Hugh~A. Barton, Jos~G. Bessems, John~C. Lipscomb, and
	Kannan Krishnan.
	\newblock Case study illustrating the {WHO} {IPCS} guidance on characterization
	and application of physiologically based pharmacokinetic models in risk
	assessment.
	\newblock {\em Regulatory Toxicology and Pharmacology}, 66(1):116--129, June
	2013.
	
	\bibitem{IPCS_2010}
	{International Programme on Chemical Safety (IPCS)}.
	\newblock Characterization and {Application} of {Physiologically} {Based}
	{Pharmacokinetic} {Models} in {Risk} {Assessment}.
	\newblock Harmonization {Project} {Document}~9, World Health Organization
	(WHO), 2010.
	
	\bibitem{graham_partition_2012}
	Helen Graham, Mike Walker, Owen Jones, James Yates, Aleksandra Galetin, and
	Leon Aarons.
	\newblock Comparison of in-vivo and in-silico methods used for prediction of
	tissue: plasma partition coefficients in rat.
	\newblock {\em Journal of Pharmacy and Pharmacology}, 64(3):383--396, 2012.
	
	\bibitem{berezhkovskiy_volume_2004}
	Leonid~M. Berezhkovskiy.
	\newblock Volume of {Distribution} at {Steady} {State} for a {Linear}
	{Pharmacokinetic} {System} with {Peripheral} {Elimination}.
	\newblock {\em Journal of Pharmaceutical Sciences}, 93(6):1628--1640, June
	2004.
	
	\bibitem{poulin_prediction_2002}
	Patrick Poulin and Frank-Peter Theil.
	\newblock Prediction of pharmacokinetics prior to in vivo studies. 1.
	{Mechanism}-based prediction of volume of distribution.
	\newblock {\em Journal of Pharmaceutical Sciences}, 91(1):129--156, January
	2002.
	
	\bibitem{willmann_development_2007}
	Stefan Willmann, Karsten H\"ohn, Andrea Edginton, Michael Sevestre, Juri
	Solodenko, Wolfgang Weiss, J\"org Lippert, and Walter Schmitt.
	\newblock Development of a {Physiology}-{Based} {Whole}-{Body} {Population}
	{Model} for {Assessing} the {Influence} of {Individual} {Variability} on the
	{Pharmacokinetics} of {Drugs}.
	\newblock {\em Journal of Pharmacokinetics and Pharmacodynamics},
	34(3):401--431, June 2007.
	
	\bibitem{brown_physiological_1997}
	Ronald~P. Brown, Michael~D. Delp, Stan~L. Lindstedt, Lorenz~R. Rhomberg, and
	Robert~P. Beliles.
	\newblock Physiological {Parameter} {Values} for {Physiologically} {Based}
	{Pharmacokinetic} {Models}.
	\newblock {\em Toxicology and Industrial Health}, 13(4):407--484, July 1997.
	
	\bibitem{rodgers_physiologically_2005}
	Trudy Rodgers, David Leahy, and Malcolm Rowland.
	\newblock Physiologically {Based} {Pharmacokinetic} {Modeling} 1: {Predicting}
	the {Tissue} {Distribution} of {Moderate}-to-{Strong} {Bases}.
	\newblock {\em Journal of Pharmaceutical Sciences}, 94(6):1259--1276, June
	2005.
	
	\bibitem{rodgers_physiologically_2006}
	Trudy Rodgers and Malcolm Rowland.
	\newblock Physiologically based pharmacokinetic modelling 2: {Predicting} the
	tissue distribution of acids, very weak bases, neutrals and zwitterions.
	\newblock {\em Journal of Pharmaceutical Sciences}, 95(6):1238--1257, June
	2006.
	
	\bibitem{heinemann_standard_1999}
	Axel Heinemann, Friedel Wischhusen, Klaus P\"uschel, and Xavier Rogiers.
	\newblock Standard liver volume in the caucasian population.
	\newblock {\em Liver Transplantation and Surgery}, 5(5):366--368, 1999.
	
	\bibitem{valetin_basic_2002}
	J.~Valetin.
	\newblock Basic {Anatomical} and {Physiological} {Data} for {Use} in
	{Radiological} {Protection}: {Reference} {Values}.
	\newblock Technical Report~89, International Commission on Radiological
	Protection (ICRP), 2002.
	
	\bibitem{brill_mdz_pbpk_2016}
	MJE Brill, PAJ VÃ¤litalo, AS~Darwich, B~van Ramshorst, HPA van Dongen,
	A~Rostamiâ€“Hodjegan, M~Danhof, and CAJ Knibbe.
	\newblock Semiphysiologically based pharmacokinetic model for midazolam and
	cyp3a mediated metabolite 1-oh-midazolam in morbidly obese and weight loss
	surgery patients.
	\newblock {\em CPT: Pharmacometrics \& Systems Pharmacology}, 5(1):20--30,
	2016.
	
	\bibitem{osp_suite}
	Open Systems~Pharmacology (OSP).
	\newblock {OSP} {Suite} - {Version} 7.1,
	(http://www.open-systems-pharmacology.org/), 2017.
	
\end{thebibliography}
